Flexibility of Networks: a new measure for network design space analysis?

Flexibility is often claimed as a competitive advantage when proposing new network designs. However, most proposals provide only qualitative arguments for their improved support of flexibility. Quantitative arguments vary a lot among different proposals. A general understanding for flexibility is not yet clearly defined, leaving it to the reader to draw the right conclusions based on background information. The term flexibility is commonly defined as the ability to adapt to changes. For networks, flexibility would refer to the ability to adapt the available network resources, such as flows or topology, to changes of design requirements, e.g., shorter latency budgets or different traffic distributions. Recent concepts such as Software Defined Networking, Network Virtualization and Network Function Virtualization have emerged claiming to provide more flexibility in networks. Nevertheless, a deeper understanding of what flexibility means and how it could be quantified to compare different network designs remains open. In this paper, we ask whether flexibility can be a new measure for network design space analysis. As it is quite challenging to formulate a flexibility measure that covers all network aspects, we propose an initial set of flexibility aspects to start grounding guidelines. Our initial selection is backed up by an analysis of Software Defined Networking, Network Virtualization and Network Function Virtualization for their support of the selected flexibility aspects. Our research methodology is based on a systematic approach that leads to network design guidelines with respect to flexibility.

==> graphs.tex <==
\section{How to make your network flexible?}

In order to serve dynamically varying user demands, network need to become flexible. As already mentioned, hopefully, in the previous sections, flexibility can be quantified in multiple dimensions. In this section, we want to carry out how to apply the perceived insights in flexibility in order to make a network more flexible. When quantifying the flexibility of an existing network, the used technologies and the underlying network topology have the main impact. Accordingly, having quantified a network, an operator has two possibilities in order to improve flexibility. The operator can upgrade the available technologies, extend the network topology, or it can do both partly/completely.

\subsection{Upgrading/changing technologies}
Upgrading/changing a technology depends on the flexibility of the currently deployed technologies and their interdependency. For instance, partly changing from IPv4 to IPv6 would need gateways that translate between both protocols. Here, network virtualization can be beneficial. For instance, a gateway, which runs in software, can ''easily'' deployed. Combining this with SDN would allow to adapt the steering flexibly. 

\subsection{Upgrading network topology}
Meshed vs star networks. A meshed network may be more flexible in terms of resilience, however, in case of distributed protocols, the signaling overhead may even be larger. A star is sufficient for supporting, e.g., multi casting. A use case dependency can be seen!

\subsection{How flexible is your network?} Can this be quantified based on the used technologies, the network graph, and the interconnections between network nodes. Which role do the demands play? Are there two metrics, a demand dependent and a demand independent. If we have, for example, a split architecture where the edges are flexible and the core is tunnel based, thus performance oriented inflexible, the whole architecture is still flexible in terms of needed demands. If we look at a network and see different types of nodes, does the flexibility only depend on the arrangement of the nodes, i.e., the optimal placement?

\subsection{Abstract analysis of demands/uses cases}
Besides investigating how to improve the flexibility of a network, the needed flexibility may also play a key role. For example, if demands in terms of footprints, data rates, latencies over time are static, a network architecture has to provide just one setup. However, the future evolution of the demands may also need to be integrated. This means that the probability that the demands change in the future have to be integrated. This could lead to stochastical demands ... what happens if ...
